Best Arm Identification in Restless Markov Multi-Armed Bandits

We study the problem of identifying the best arm in a multi-armed bandit environment when each arm is a time-homogeneous and ergodic discrete-time Markov process on a common, finite state space. The state evolution on each arm is governed by the arm's transition probability matrix (TPM). A decision entity that knows the set of arm TPMs but not the exact mapping of the TPMs to the arms, wishes to find the index of the best arm as quickly as possible, subject to an upper bound on the error probability. The decision entity selects one arm at a time sequentially, and all the unselected arms continue to undergo state evolution ({\em restless} arms). For this problem, we derive the first-known problem instance-dependent asymptotic lower bound on the growth rate of the expected time required to find the index of the best arm, where the asymptotics is as the error probability vanishes. Further, we propose a sequential policy that, for an input parameter $R$, forcibly selects an arm that has not been selected for $R$ consecutive time instants. We show that this policy achieves an upper bound that depends on $R$ and is monotonically non-increasing as $R\to\infty$. The question of whether, in general, the limiting value of the upper bound as $R\to\infty$ matches with the lower bound, remains open. We identify a special case in which the upper and the lower bounds match. Prior works on best arm identification have dealt with (a) independent and identically distributed observations from the arms, and (b) rested Markov arms, whereas our work deals with the more difficult setting of restless Markov arms.

==> intro.tex <==
\section{Introduction}
The multi-arm bandit problem exemplifies the exploration-exploitation tradeoff and forms  an active research topic in online machine learning and  information theory. This problem find numerous applications in digital auctions, ad placements, clinical trials, resource allocations, gambling, and many more; see \cite{lattimore2020bandit} for details. A multi-arm bandit problem is characterized by  $K$ arms in which   each arm {\color{red}$a$} is associated to an unknown reward distributions {\color{red}$\psi_a$}. These arms are independent of one another in the sense that obtaining a reward of one arm does not provide the decision maker with any information about other arms. At each point in time, a decision maker must explore the environment to find which arm is the best and subsequently pulls it to obtain a sample from the associated distribution. The difference between the highest possible reward and the reward obtained by the decision maker at a particular time slot is known as the {\em instantaneous regret}.  The aim of the decision maker is to minimize the {\em cumulative regret}, which is the sum of the instantaneous regrets over all time slots. This problem is known as {\em regret minimization}. Regret minimization under various settings have been studied in the literature; see \cite{lattimore2020bandit} for details.

The study of regret minimization is useful for applications such as ad placements or digital auctions in which  the objective is to maximize the overall profit. However, in applications like clinical trials, our objective is to identify the best drug as fast as and as accurately as possible. The problem of identifying the arm with highest reward is known as the {\em best arm identification} or {\em pure exploration} problem in the literature. The accuracy of the best arm identification problem generally increases with the number of permissible time steps. Two types of best arm identification problems are studied in the literature. The first one is known as the {\em  fixed-confidence problem}, where the objective is to identify the best arm with accuracy above a given threshold in the minimum number of time slots. The second one is the {\em fixed-budget problem}, where the objective is to identify the best arm as accurately as possible in a given fixed number of time slots. %, i.e., the number of time-slots are fixed and no limit on accuracy. 
In our paper, we focus on a fixed confidence best arm identification problem.

In the standard multi-arm bandit problem, we assume that the rewards or observations from each arm  are generated  independently and according to the same   distribution. {\color{red}Motivated by the Google PageRank algorithm, in our problem we assume  that the arm observations follow a discrete-time, finite-state Markov process.} Accordingly, we study a best arm identification problem for this Markov chain multi-arm bandit problem in the fixed-confidence setting.  Note that there are many works which study the Markov chain multi-arm bandit problem under the regret minimization setting; see  for example \cite{bubeck2012regret}.

In a Markov chain multi-arm bandits, similar to the standard multi-arm bandit problem, there are $K$ arms. But, in the standard multi-arm bandit problem, the rewards of an arm are  generated from an independent and identical distribution ({\em i.i.d.}) process. In contrast, in a Markov chain multi-arm bandits, the rewards of an arm follow an ergodic Markov chain/process. We assume that the arms are independent of each other, i.e., obtaining a reward of one arm doesn't provide any information about the other arms. Let $\mathcal{S}$ denotes the  state-space of given arms and  $\pmb{\mu_a}=\{\mu_{a}(s):s\in \mathcal{S}\}$ denotes the stationary distribution of Arm $a$. Then, for a given function $f:\mathcal{S} \to \mathbb{R}$, Arm $a$'s average reward is $\sum_{s\in\mathcal{S}}f(s)\mu_{a}(s)$. A decision maker, whose aim is to identify the arm with the highest average reward, samples the arms sequentially, one at a time. If sufficiently confident about the arm with the highest reward, the decision maker stops sampling. Otherwise, the decision maker samples the arms according to an optimal policy. The optimal policy is a policy that identifies the best arm as soon as possible with the probability of error below a given value. We aim to identify the asymptotic growth rate of the optimal policy stopping time as a function of the error probability, where the asymptotics is as the error probability goes to zero.

Two types of multi-arm bandits are considered in the literature. One of them is the rested Markov multi-arm bandit, in which the Markov process of any given arm evolves by one-time step only when the arm is selected  and does not evolve otherwise. The other one is the restless Markov multi-arm bandit, in which the Markov process of each arm continues to evolve whether or not the arm is selected. Best arm identification under the rested multi-arm bandit has been studied in \cite{moulos2019optimal}.  Our work considers the best arm identification in a challenging Markov setting, i.e., the best arm identification in a restless multi-arm bandit. The restless multi-arm bandit is challenging because in the rested case, the state of the sampled arm depends only on its previous state observed, whereas in the restless case, the state of the sampled arm also depends on the time elapsed since the arm was previously selected in addition to the previously observed state of the arm. Hence, in a restless multi-arm bandit, we need to keep track of (a) the time elapsed since each arm was previously selected (called the arm’s \textit{delay}), and (b) the state of each arm as observed at its previous selection time (called the \textit{last observed state} of the arm). These arm delays and last observed states are superfluous in the standard multi-arm bandits because the sampled arm rewards are independent of time and its previously observed states. The arm delays are superfluous in the rested multi-arm bandits because the arm rewards don't evolve if we don't select the arm. 

In our work, similar to \cite{karthik2021detecting}, we assume that the transition probability matrices are known up to a permutation, but the exact matching between the arms and its corresponding transition matrix is unknown. We also assume that the common state space of the transition matrices is finite. Despite these assumptions, many difficulties related to restless arms remain. Section \ref{sec:contribtion}  highlights the contributions of our work. The case
when transition probabilities are unknown is beyond the scope of this paper and is currently under study.

In our work, we derive a lower bound for the expected stopping time of a general best arm identification problem in restless multi-arm bandits, and the lower bound is based on a solution of a sup-min optimization problem, where the supremum is over all possible state-action occupancy measures; see Proposition \ref{prop:lower_bound} for details. Due to the countably infinite nature of the state-action space, it is not clear whether the supremum in the lower bound is attainable or not. To counter the difficulty, earlier works \cite{karthik2021detecting,karthik2021learning} assume a trembling hand parameter model. In our paper, to counter the difficulty, we assume the restless multi-arm bandits with delay constraints. In restless multi-arm bandits with delay constraints, the state-action space is finite and is practically implementable. We derive a lower bound for the delay constrained restless multi-arm bandits and propose a matching policy that achieves the lower bound. 


\subsection{Related work}
The seminal work of \cite{lai1985asymptotically} studied the regret minimization in multi-arm bandit with \textit{i.i.d.} processes. Later \cite{anantharam1987asymptotically} extended the regret minimization problem to the more general Markov multi-arm bandit. See \cite{bubeck2012regret} for an extensive survey of the regret minimization problems. As we mentioned earlier, the best arm identification is the alternative object in the multi-arm bandit problems. \cite{mannor2004sample,garivier2016optimal} derived the lower bound on the sample complexity of best arm identification in multi-arm bandit with \textit{i.i.d.} processes. Many algorithms are proposed to match the lower bounds. Some of the algorithms  are action-elimination algorithms \cite{even2002pac,karnin2013almost}, upper confidence bound (UCB) algorithms \cite{jamieson2014lil,audibert2010best} and  lower and upper confidence bound (LUCB) algorithms \cite{kalyanakrishnan2012pac,kaufmann2013information} etc. The best arm identification in multi-arm bandit with \textit{i.i.d.} process is settled in \cite{garivier2016optimal} with a change of measure based lower bound and a matching track and stop algorithm. 

\cite{moulos2019optimal} extended the best arm identification in multi-arm bandit with \textit{i.i.d.} process to the Markov chain process. In particular, \cite{moulos2019optimal} studied the best arm identification in rested Markov chains, whereas our work focuses on restless Markov chain. For the rested Markov chain case, \cite{moulos2019optimal} derived the upper and lower bounds, which differ by a constant multiplicative factor. \cite{karthik2020learning,karthik2021detecting,karthik2021learning} also studied the multi-arm bandit with Markov chain processes under the fixed confidence setting. Similar to our work, \cite{karthik2021detecting,karthik2021learning} focused on restless multi-arm bandit, whereas \cite{karthik2020learning} focused on rested multi-arm bandit. But, the primary objective in \cite{karthik2021detecting,karthik2021learning} is to identify an anomalous (odd) arm, whereas our work focuses on the best arm identification problem. The second difference is to overcome the challenges in restless multi-arm bandit, \cite{karthik2021detecting,karthik2021learning} assumes a trembling hand model motivated from a certain visual science experiment. In contrast, we focus on restless multi-arm bandits with delay constraints. \cite{karthik2021detecting,karthik2021learning} derived matching lower and upper bounds for the odd arm identification in restless multi-arm bandit. \cite{karthik2021detecting} assumes that the transition probability matrices are known to the decision maker, and \cite{karthik2021learning} extends it to the unknown transition probability case. 

The recent works \cite{deshmukh2018controlled,deshmukh2021sequential,prabhu2020sequential} studied the more general problems of
sequential hypothesis testing in multi-armed bandits, special cases of which are the problems of best arm identification and odd arm identification, in the context of \textit{i.i.d.} observations from each arm. The multi-arm bandit problems are also extended to more general cases like correlated bandits \cite{gupta2021best},  cascaded bandits \cite{zhong2020best} and bandits with switching costs \cite{dekel2014bandits} etc.


\subsection{Contributions}\label{sec:contribtion}
In this paper, we study the best arm identification in restless  multi-arm bandit problem and make the following technical contributions:
\begin{itemize}
	\item[--] We derive a lower bound for the general best arm identification in restless multi-arm bandit problem (Proposition \ref{prop:lower_bound}) expected stopping time. Our lower bound is instance-specific, i.e., the lower bound depends on the transition probability matrices of the given problem instance. 
	\item[--] Our lower bound for the general best arm identification in restless multi-arm bandit problem is a solution of a sup-min optimization problem, where the supremum is over all possible state-action occupancy measures with certain constraints; see \eqref{eq:T_a^{star}} for details. Due to the countably infinite nature of the state-action space, it is not clear whether the supremum in the lower bound is attainable or not. To counter this difficulty, we consider the restless multi-arm bandits with delay constraints, i.e., an arm is forcibly selected if its delay reached maximum value $R$; see Section \ref{sec:achievability} for details. In restless multi-arm bandits with delay constraints, the state-action space is finite and is practically implementable.
	As far as we know, this is the first work to consider the restless multi-arm bandit with the delay constraints.
	\item[--] For the best-arm identification in restless multi-arm bandit with the delay constraints, we derive the expected time taken by the decision
	maker to identify the index of the best arm with the probability of error at most a given pre-specified  value $\epsilon$. Similar to the other fixed confidence problem earlier works, the expected time is  $\Theta(\ln(1/\epsilon))$. We give
	a precise characterization of the best (smallest) constant multiplying $\ln(1/\epsilon)$ and the constant is $1/T_R^*(C)$, which is a function of the transition probabilities and delay constraint $R$, see \eqref{eq:T-R-star-C} for details. 
	\item[--]  Note that for a given delay constraint $R$, $\ln(1/\epsilon)/T_R^*(C)$ also works as an upper bound for the  general best arm identification in restless multi-arm bandit problem expected stopping time. We also show that $T_R^*(C)$ is an increasing function of the delay constraint $R$ and $T_R^*(C)$ is bounded by the $T^*(C)$ in \eqref{eq:T_a^{star}}. We are expecting that $T_R^*(C)$ converges to $T^*(C)$ and is still under study. We showed that for some special transition probability matrices, $T_R^*(C)$ is indeed equal to $T^*(C)$. 
	\item[--] By following the trembling hand approach in \cite{karthik2021detecting}, we also give an another upper bound for the  general best arm identification in restless multi-arm bandit problem expected stopping time.
	%\item[--] {\color{red}Simulations}
\end{itemize}

\subsection{Paper organization}
The rest of this paper is organized as follows. In Section \ref{sec:notations_prel}, we briefly discuss the problem setup and mention the notations that we use throughout the paper.
In Sections \ref{sec:delays-last-observed-states} and \ref{sec:llr}, we provide some preliminaries on delays, last observed states and  MDPs and discuss the log-likelihoods and log-likelihood ratios. These are useful in deriving our lower and upper bounds. 
In Section \ref{sec:lower_bound}, we present a lower bound on the expected time to identify the best arm as a function of the error probability for the general setting of restless Markov arms. In Sections \ref{sec:achievability} and \ref{sec:upper_bound}, to overcome the difficulties in restless multi-arm bandits, we introduce delay constrained restless multi-arm bandits. For this delay constrained restless multi-arm bandits, we derive a lower bound, and propose a policy that achieves the lower bound. All the proofs are relegated to the Appendices.







==> setting.tex <==
\section{setting}
Write something about best arm identification problem with restless Markov chains.

We consider a multi-arm bandit problem with $K$ arms $\{1,2,...,K\}$ ($=[K]$), where each arm represents a {\color{red}unique} Markov chain with finite state space $\mathcal{S}$. Let $X_t^a$ denotes the state of Arm $a$ at time $t$ and $P_a$ denotes the transition matrix of Arm $a$. {\color{red}We assume that $P_a$ is ergodic for every $a\in[K]$.} Let $\mathbf{\mu_a}=\{\mu_{a,1},\mu_{a,2},...,\mu_{a,|\mathcal{S}|}\}$ denotes the stationary distribution of Arm $a$, and is completely characterized by the transition matrix $P_a$. Let a non-constant real-valued function $f:\mathcal{S}\rightarrow \mathbb{R}$ denotes the reward of the states and $\nu_a=\sum_{s\in\mathcal{S}}f(s)\mu_{a,s}$ denotes the ergodic mean reward of Arm $a$. {\color{red}Without loss of generality (WLOG), we assume that $\nu_1 > \nu_2 \geq \nu_3 \geq ... \geq \nu_K$. } Let $a^*$ be the arm with highest ergodic mean reward, i.e., $a^*=\arg\max_a\nu_a$. In our work, we assume that there is only one arm with highest mean reward, i.e., $\nu_{a^*}>\nu_a$, $\forall a\neq a^*$.


Let $\mathcal{C}=\{P_{\sigma(1)},P_{\sigma(2)},...,P_{\sigma(K)}: \sigma \text{ is a permutation}\}$ denotes the all possible configurations of arms and $\mathcal{C}_a$ denotes the all configurations such that $\sigma(a)=a^*$, i.e., $\mathcal{C}_a=\{P_{\sigma(1)},P_{\sigma(2)},...,P_{\sigma(K)}: \sigma(a)=a^*\}$. Let $c\in \mathcal{C}$ be an unknown configuration / problem instance is given to us. We aim to design efficient algorithms to fine the best arm for the given unknown configuration $c\in \mathcal{C}$.

Our algorithm proceeds in rounds as follows:
\begin{itemize}
    \item In each round, the algorithm selects an arm and observes the reward associated with it. Let $A_n$ denotes the arm selected at round $n\in\mathbb{N}$ and $\bar{X}_n$ denotes the reward observed, i.e., $\bar{X}_n=X_n^{A_n}$ for restless multi-arm bandits. Note that the algorithm selects an arm at time $n$ based on its past selected arms $A_0^{n-1}$ and their observations $\bar{X}_0^{n-1}$.
    \item Based on all its selected arm $A_0^{n}$ and their observations $\bar{X}_0^{n}$, the algorithm decides whether to terminate or to proceed to next round.
    \item If the algorithm terminates, it returns an arm $\hat{a}\in[K]$ as the best arm.
\end{itemize}

{\color{blue}Write something about $\delta-$pac algorithms etc.,}

%the algorithm makes two decisions $\{\textit{continue, stop}\}$ based on its past observations. 

==> srs-policies-and-ergodicity.tex <==
\section{Stationary Randomised Strategies and a Key Ergodicity Property}

Under an arbitrary policy $\pi$, the action $A_t$ may, in general, be chosen based on the history $\mathcal{F}_t$ for each $t\geq K$. In the special case when $A_t$ is chosen based only on the current state $(\underline{d}(t), \underline{i}(t))$ for all $t\geq K$, the controlled Markov process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is, in fact, a Markov process. To see this, note that
\begin{align}
&P_C^\pi(\underline{d}(t+1)=\underline{d}',\underline{i}(t+1)=\underline{i}'\mid \{(\underline{d}(s),\underline{i}(s)), \ K\leq s \leq t\})\nonumber\\
&=\sum_{a=1}^{K}\ P_C^\pi(\underline{d}(t+1)=\underline{d}',\underline{i}(t+1)=\underline{i}', A_t=a\mid \{(\underline{d}(s),\underline{i}(s)), \ K\leq s \leq t\})\nonumber\\
&\stackrel{(a)}{=}\sum_{a=1}^{K}\ P_C^\pi(A_t=a\mid \{(\underline{d}(s),\underline{i}(s)), \ K\leq s \leq t\}) \cdot Q_{C}(\underline{d}', \underline{i}'|\underline{d}(t), \underline{i}(t), a)\nonumber\\
&=\sum_{a=1}^{K}\ P_C^\pi(A_t=a\mid \underline{d}(t),\underline{i}(t)) \cdot Q_{C}(\underline{d}', \underline{i}'|\underline{d}(t), \underline{i}(t), a)\nonumber\\
&=P_C^\pi(\underline{d}(t+1)=\underline{d}',\underline{i}(t+1)=\underline{i}'\mid \underline{d}(t),\underline{i}(t)),
\label{eq:A_t_is_selected_based_on_d(t)_i(t)_only}
\end{align}
where $(a)$ above follows from \eqref{eq:controlled_markov_chain}.

Call $\pi$ a {\em stationary randomised strategy} (or SRS policy) if there exists $\lambda=\bigotimes _{(\underline{d},\underline{i})\in\mathbb{S}} \lambda(\cdot|\underline{d},\underline{i})$, with the component $\lambda(\cdot|\underline{d},\underline{i})$ being a probability distribution on $\mathcal{A}$ for each $(\underline{d},\underline{i})\in \mathbb{S}$, such that 
\begin{equation}
P_C^\pi(A_t=a\mid \mathcal{F}_t)=\lambda(a|\underline{d}(t),\underline{i}(t)) \quad \forall \ t\geq K.
\label{eq:SRS_policy}
\end{equation}
Let the SRS policy in \eqref{eq:SRS_policy} be denoted explicitly as $\pi^\lambda$, and let $\Pi_{\textsf{SRS}}$ denote the space of all SRS policies. If the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is ergodic under the SRS policy $\pi^{\lambda}$, it possesses a unique stationary distribution which we denote by $\mu^\lambda=\{\mu^\lambda(\underline{d}, \underline{i}):\ (\underline{d}, \underline{i})\in \mathbb{S}\}$. Further, we write 
\begin{equation}
\nu^\lambda(\underline{d}, \underline{i}, a) \coloneqq \mu^\lambda(\underline{d}, \underline{i}) \ \lambda(a|\underline{d}, \underline{i}), \quad (\underline{d}, \underline{i})\in \mathbb{S}, \ a\in \mathcal{A},
\label{eq:ergodic_state_action_occupancy_measure}
\end{equation}
to denote the {\em ergodic state-action occupancy} measure under $\pi^\lambda$. We write $\pi^{\textsf{unif}}$ to denote the SRS policy defined by
\begin{equation}
\lambda_{\textsf{unif}}(a|\underline{d}, \underline{i})=\frac{1}{K}, \quad a\in \mathcal{A}, \ (\underline{d}, \underline{i})\in \mathbb{S}.
\label{eq:unif-SRS-policy}
\end{equation}

The below result demonstrates that the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is ergodic under $\pi^{\textsf{unif}}$.
\begin{lemma}
\label{lemma:ergodicity-under-unif-SRS-policy}
For each $C\in \mathcal{C}$, the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is ergodic under the SRS policy $\pi^{\textsf{unif}}$ and under the TPMs assignment $C$.
\end{lemma}
\begin{IEEEproof}
See Appendix \ref{appndx:proof-of-lemma-ergodicity-under-unif-SRS-policy}.
\end{IEEEproof}
As a consequence of Lemma \ref{lemma:ergodicity-under-unif-SRS-policy}, the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ has a unique stationary distribution, say $\mu_{C}^{\textsf{unif}}=\{\mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i}): (\underline{d}, \underline{i})\in \mathbb{S}\}$, under the SRS policy $\pi^{\textsf{unif}}$ and under the TPMs assignment $C$. We note that $\mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i})>0$ for all $(\underline{d}, \underline{i})\in \mathbb{S}$. Let
\begin{align}
\nu_{C}^{\textsf{unif}}(\underline{d}, \underline{i}, a) &\coloneqq \mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i})\cdot \lambda_{\textsf{unif}}(a|\underline{d}, \underline{i})\nonumber\\
&= \frac{\mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i})}{K}, \quad (\underline{d}, \underline{i})\in \mathbb{S}, \ a\in \mathcal{A},
\label{eq:ergodic-state-action-under-unif}
\end{align}
denote the corresponding ergodic state-action occupancy measure. 



